TUNA: Tuning Unstable and Noisy Cloud Applications

Autotuning plays a pivotal role in optimizing the performance of systems, particularly in large-scale cloud deployments. One of the main challenges in performing autotuning in the cloud arises from performance variability. We first investigate the extent to which noise slows autotuning and find that as little as $5\%$ noise can lead to a $2.5$x slowdown in converging to the best-performing configuration. We measure the magnitude of noise in cloud computing settings and find that while some components (CPU, disk) have almost no performance variability, there are still sources of significant variability (caches, memory). Furthermore, variability leads to autotuning finding unstable configurations. As many as $63.3\%$ of the configurations selected as "best" during tuning can have their performance degrade by $30\%$ or more when deployed. Using this as motivation, we propose a novel approach to improve the efficiency of autotuning systems by (a) detecting and removing outlier configurations and (b) using ML-based approaches to provide a more stable true signal of de-noised experiment results to the optimizer. The resulting system, TUNA (Tuning Unstable and Noisy Cloud Applications) enables faster convergence and robust configurations. Tuning postgres running mssales, an enterprise production workload, we find that TUNA can lead to $1.88$x lower running time on average with $2.58x$ lower standard deviation compared to traditional sampling methodologies.

==> deleted.tex <==
\label{sec:FullSystemVariance}
\subsubsection{End-to-End System Performance}
\input{figures/FullSystemVariability}
The components that still show significant variability are unfortunately still important for end-to-end systems.
Memory and Cache are key components for almost every large system that runs today, and the impact of the OS depends more on the implementation.

Two full systems that we profiled are Postgres using \texttt{pgbench} and Redis using \texttt{redis\-test}.
We report the results of our benchmarking in Figure~\ref{fig:full_system_variability}.
We find that the \texttt{redis-test} benchmarks \texttt{LPUSH} and \texttt{SET} have a CoV of $3.21\%$ and $3.92\%$ respectively and the \texttt{pgbench} read/write benchmark on a small database and a large database had a CoV of $4.73\%$ and $1.38\%$ respectively.
One notable takeaway is that as Postgres moves from being memory resident in the small workload to having a data set multiple times larger than the memory and becoming disk-resident, the CoV decreases.
Additionally, it is also important to note the long tails, especially on the lower end of performance.
The memory resident workloads each degrade up to $47.1-50.5\%$ from the mean, while the large Postgres workload degrades up to $37.8\%$ from the mean, once again showing more stable performance.
If we simply remove the bottom percent of samples, the three memory resident workloads still experience $18.5 - 21.5\%$ maximal performance loss from the mean, and the disk resident workload only see up to $11.8\%$ performance loss.

\TakeawayBox{Full end-to-end systems are significantly impacted by performance variability, especially if they are heavily dependent on memory performance. }






\subsection{Tuning in the Cloud}
To quantify the impacts of the variability in the cloud on ML-based knob configuration tuning, we will run a series of measurement-based case studies.
First, we will run a series of tuning runs using state-of-the-art methods in the cloud to investigate the impacts of interference.
Specifically, we will investigate the performance anomalies in configurations seen during tuning, as well as the best-learned configuration.
Secondly, we will investigate the impacts of performance noise on the convergence rate of tuning.

For all of our experiments, we will use SMAC~\cite{SMAC3}, a state-of-the-art Bayesian optimization (BO) based optimizer as it has been shown to outperform alternatives~\cite{FacilitatingDBMSTuning, Llamatune}.
For our SuT, we will target Postgres 16.1 running TPC-C~\cite{tpcc}.
The optimizer will run with $10$ initialization points (similar to prior works~\cite{FacilitatingDBMSTuning, Llamatune}) unless stated otherwise.
The initialization points consist of $9$ configurations which are random, but identical across runs, and the default configuration.

Once the tuning run has been completed, we select the best configuration seen, based on the performance seen during tuning, and deploy it to a set of $10$ new machines.
We will refer to this as our test cluster.
We use this test cluster as a way to represent the possible performance one could see when deploying this configuration in production when deploying from a test setup to a production setup.


==> figures/FullSystemVariability.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/ViolinFullSystem.pdf}
    \Description[Timeline.]{Timeline.}
    \caption{The variance of benchmarks targeting \redis and \postgres}
    \label{fig:full_system_variability}
\end{figure}

==> figures/StableResultsTable.tex <==
\begin{table*}[]
\begin{tabular}{rr|llll|llll}
\multicolumn{1}{l}{} &
  VM Lifespan &
  \multicolumn{4}{c|}{Short} &
  \multicolumn{4}{c}{Long} \\
\multicolumn{1}{l}{} &
  Region &
  \multicolumn{2}{c}{West} &
  \multicolumn{2}{c|}{East} &
  \multicolumn{2}{c}{West} &
  \multicolumn{2}{c}{East} \\
\multicolumn{1}{l}{} &
  Metric &
  \multicolumn{1}{c}{Mean} &
  \multicolumn{1}{c|}{\textbf{CoV}} &
  \multicolumn{1}{c}{Mean} &
  \multicolumn{1}{c|}{\textbf{CoV}} &
  \multicolumn{1}{c}{Mean} &
  \multicolumn{1}{c|}{\textbf{CoV}} &
  \multicolumn{1}{c}{Mean} &
  \multicolumn{1}{c}{\textbf{CoV}} \\ \cline{2-10} 
\multirow{5}{*}{\rotatebox[origin=c]{90}{Benchmark}} &
  CPU Matrix Multiply (Ops/s) &
  20,603 &
  \multicolumn{1}{l|}{\textbf{0.71\%}} &
  20,598 &
  \textbf{0.71\%} &
  20,590 &
  \multicolumn{1}{l|}{\textbf{0.34\%}} &
  20,554 &
  \textbf{0.22\%} \\
 &
  Disk Sequential Read (IOPS) &
  5097.8 &
  \multicolumn{1}{l|}{\textbf{0.06\%}} &
  5097.7 &
  \textbf{0.04\%} &
  5096.8 &
  \multicolumn{1}{l|}{\textbf{0.08\%}} &
  5096.3 &
  \textbf{0.03\%} \\
 &
  Disk Sequential Write (IOPS) &
  5097.9 &
  \multicolumn{1}{l|}{\textbf{0.07\%}} &
  5097.8 &
  \textbf{0.10\%} &
  5097.0 &
  \multicolumn{1}{l|}{\textbf{0.03\%}} &
  5096.5 &
  \textbf{0.03\%} \\
 &
  Disk Random Read (IOPS) &
  5097.7 &
  \multicolumn{1}{c|}{\textbf{0.19\%}} &
  5097.6 &
  \textbf{0.36\%} &
  5096.8 &
  \multicolumn{1}{l|}{\textbf{0.04\%}} &
  5096.3 &
  \textbf{0.03\%} \\
 &
  Disk Random Write (IOPS) &
  5097.0 &
  \multicolumn{1}{c|}{\textbf{0.36\%}} &
  5097.0 &
  \multicolumn{1}{c|}{\textbf{0.16\%}} &
  5096.1 &
  \multicolumn{1}{l|}{\textbf{0.07\%}} &
  5095.3 &
  \textbf{0.04\%}
\end{tabular}
\caption{Performance results showing the performance stability of CPU and Disk cloud system components in Azure. Note the extremely low CoV on all of these measurements.}
\label{table:CloudStability}
\end{table*}

==> related_work.tex <==
% MOVED TO CLOUD STUDY
%\noindent\textbf{Performance Variability.}
%Hardware and cloud system variability has been studied for many decades in many applications of system design \cite{TamingPerformanceVariability, CpuCorePerfVariance, HPCVariability, SSDPerfTransperency, GPUVariance}. 
%Recent work has studied hardware variability that can lead to gray failures \cite{GrayFailure1, GrayFailure2, OriginalGray}.
%Many types of systems attempt to be agnostic to absolute system performance or have solutions that do not need profiling.
%One such system is MapReduce which duplicates work to avoid stragglers~\cite{MapReduce}.

% Double check to make sure that we have these citations
%With the rise in popularity of cloud computing, there has been work to profile performance issues in cloud environments~\cite{CloudIOVariance, EC2PerfVariance, VL2CloudNetworks}.
%Shortly after the inception of cloud environments it became clear that the systems are not homogeneous.
%\citet{CloudMoreForMoney} proposes a method of placement gaming to exploit the heterogeneity of VMs in clouds to gain up to 34\% performance improvement.
%There has also been work to determine the type of workload that is present on collocated VMs~\cite{NoisyNeighborAttack}.
%We argue that while further advancements in isolation and scheduling are of course useful and important, interference ("noisy neighbors") will continue to be an important issue for systems developers and operators, particularly those working with shared infrastructure, and hence any system that intends to run in the cloud needs to be capable of addressing increased noise.

\noindent\textbf{Interference Aware Systems.}
There has been a lot of work in the context of systems that attempt to mitigate interference through placement strategies.
In the cluster scheduling space, there has been \texttt{PARTIES}~\cite{PARTIES}, \texttt{FIRM}~\cite{FIRM}, and \texttt{Resource Central}~\cite{ResourceCentral}.
Similar concepts have also been deployed in the hypervisor in works such as \texttt{ppXen}~\cite{ppXen}, and \texttt{AaFS}~\cite{AffinityAwareScheduling}.
The HPC community has also worked on interference-aware systems, mostly in the context of networking~\cite{HPCInterference, NoiseInTheClouds}.

\noindent\textbf{Heavy Interference Detection.}
In the context of software testing, there has been work to detect outliers caused by performance regression in the cloud rather than the system design.
Some works are as simple as taking more samples across machines~\cite{howbadistesting}, or better test orderings~\cite{testordering}.
Other works have taken this a step further, and integrated metrics into outlier detection~\cite{outlierdetection1, outlierdetection2}, however, there is no work we are aware of that goes beyond using metrics detection.
Finally, there have been works to build models to do root cause analysis for platform providers~\cite{noisyneighborrootcause}.
While this is certainly useful, we feel it is complimentary and orthogonal to our work.

%MOVED TO BACKGROUND
%\noindent\textbf{Systems Tuning.}
%There have been many works that do ML-based tuning of various systems such as in tuning in storage systems~\cite{storagetuning,  HPCStorageTuning}, cluster scheduling~\cite{clustertuning}, distributed systems~\cite{SparkTuning, SparkTuning2}, and OS Tuning~\cite{OSTuning}.
%One of the most popular areas for system tuning has been DBMS.
%Many of the most successful systems use some variant of Bayesian Optimization (BO) tuning~\cite{Ottertune, Llamatune, OtterTuneRealWorld} for their optimizer, as it can find the optimum in fewer evaluations.
%Reinforcement learning (RL)~\cite{QTune, CDBTune} has also been used for this task, yet RL often requires an initial training phase which can be time-consuming.
%CDBTune focuses on parallelizing training in a cloud environment, however, it does not address the noise that is inherent~\cite{CDBTune}.
%There have been other works expanding further on this idea to improve convergence using randomized projections~\cite{Llamatune}, language models~\cite{gpttuner, DBBert}, Reinforcement Learning~\cite{QTune, CDBTune}.
%While there has been a lot of work in this area, no prior work that we are aware of has focused on the stability of configurations.
%We argue that for these systems to be reliable in production, the tuning system needs to account for the variance between machines, and the noise of the cloud environment.

%\noindent\textbf{Trade-off between Mean and Variance.}
%The trade-off between mean and variance has been explored in finance in the context of portfolio management~\cite{MarkowitzMeanVariance}.
%This has been further expanded into using many other metrics such as semi-variance~\cite{MeanSemiVariance, MeanSemiVariance2}, absolute deviation~\cite{MeanAbsoluteDeviation}, and skew~\cite{MeanVarianceSkewModel}.
%We do not deeply explore these metrics, and instead simply rely on standard deviation, leaving further metric exploration to future work.
